Search for the rare decays of $D\to h(h^{(')})e^{+}e^{-}$

We search for 15 rare decays of $D$ mesons to hadrons accompanied by an electron-positron pair $D\to h(h^{(')})e^{+}e^{-}$, based on 20.3 fb$^{-1}$ of $e^+ e^-$ collision data collected at the center-of-mass energy of 3.773 GeV with the BESIII detector at BEPCII. No significant signals are observed, and the corresponding upper limits on the branching fractions at the 90\% confidence level are determined. The sensitivities of the results are at the level of $10^{-6}$ $\sim$ $10^{-7}$. The upper limits on the branching fractions for the $D^+\to \rho^{+} e^+ e^-$, $D^+\to K^{*+} e^+ e^-$, $D^0\to K_S^0 K_S^0 e^+ e^-$, $D^0\to \pi^0 \pi^0 e^+ e^-$ and $D^0\to \eta^{\prime} e^+ e^-$ decay channels are measured for the first time. For the $D^0\to \pi^0 e^+ e^-$, $D^0\to \eta e^+ e^-$, $D^0\to \omega e^+ e^-$, $D^0\to K_S^0 e^+ e^-$, $D^+\to \pi^+ \pi^0 e^+ e^-$, $D^+\to K^+ \pi^0 e^+ e^-$, $D^+\to \pi^+ K_S^0 e^+ e^-$ and $D^+\to K^+ K_S^0 e^+ e^-$ decay channels, the upper limits on the branching fractions are determined, with an improvement of at least a factor of four compared to previous searches. The upper limits on the branching fractions for the $D^0\to \rho^{0} e^+ e^-$ and $D^0\to \phi e^+ e^-$ decay channels are set at $0.7 \times 10^{-6}$ and $4.6 \times 10^{-6}$, respectively.

==> acknowledgement_2025-12-05.tex <==
%% Saved at => 2025-12-05
\textbf{Acknowledgement}

The BESIII Collaboration thanks the staff of BEPCII (https://cstr.cn/31109.02.BEPC) and the IHEP computing center for their strong support. This work is supported in part by National Key R\&D Program of China under Contracts Nos. 2023YFA1606000, 2023YFA1606704; National Natural Science Foundation of China (NSFC) under Contracts Nos. 11635010, 11935015, 11935016, 11935018, 12025502, 12035009, 12035013, 12061131003, 12192260, 12192261, 12192262, 12192263, 12192264, 12192265, 12221005, 12225509, 12235017, 12342502, 12361141819; the Chinese Academy of Sciences (CAS) Large-Scale Scientific Facility Program; the Strategic Priority Research Program of Chinese Academy of Sciences under Contract No. XDA0480600; CAS under Contract No. YSBR-101; 100 Talents Program of CAS; The Institute of Nuclear and Particle Physics (INPAC) and Shanghai Key Laboratory for Particle Physics and Cosmology; ERC under Contract No. 758462; German Research Foundation DFG under Contract No. FOR5327; Istituto Nazionale di Fisica Nucleare, Italy; Knut and Alice Wallenberg Foundation under Contracts Nos. 2021.0174, 2021.0299, 2023.0315; Ministry of Development of Turkey under Contract No. DPT2006K-120470; National Research Foundation of Korea under Contract No. NRF-2022R1A2C1092335; National Science and Technology fund of Mongolia; Polish National Science Centre under Contract No. 2024/53/B/ST2/00975; STFC (United Kingdom); Swedish Research Council under Contract No. 2019.04595; U. S. Department of Energy under Contract No. DE-FG02-05ER41374

\textbf{Other Fund Information}

To be inserted with an additional sentence into papers that are relevant to the topic of special funding for specific topics. Authors can suggest which to Li Weiguo and/or the physics coordinator.
        Example added sentence: This paper is also supported by the NSFC under Contract Nos. 10805053, 10979059, ....National Natural Science Foundation of China (NSFC), 10805053, PWANational Natural Science Foundation of China (NSFC), 10979059, Lund弦碎裂强子化模型及其通用强子产生器研究National Natural Science Foundation of China (NSFC), 10775075, National Natural Science Foundation of China (NSFC), 10979012, baryonsNational Natural Science Foundation of China (NSFC), 10979038, charmoniumNational Natural Science Foundation of China (NSFC), 10905034, psi(2S)->B BbarNational Natural Science Foundation of China (NSFC), 10975093, D 介子National Natural Science Foundation of China (NSFC), 10979033, psi(2S)->VPNational Natural Science Foundation of China (NSFC), 10979058, hcNational Natural Science Foundation of China (NSFC), 10975143, charmonium rare decays
%% ends here %%

